Efficiency in the Serverless Cloud Paradigm: A Survey on the Reusing and Approximation Aspects

Serverless computing along with Function-as-a-Service (FaaS) is forming a new computing paradigm that is anticipated to found the next generation of cloud systems. The popularity of this paradigm is due to offering a highly transparent infrastructure that enables user applications to scale in the granularity of their functions. Since these often small and single-purpose functions are managed on shared computing resources behind the scene, a great potential for computational reuse and approximate computing emerges that if unleashed, can remarkably improve the efficiency of serverless cloud systems -- both from the user's QoS and system's (energy consumption and incurred cost) perspectives. Accordingly, the goal of this survey study is to, first, unfold the internal mechanics of serverless computing and, second, explore the scope for efficiency within this paradigm via studying function reuse and approximation approaches and discussing the pros and cons of each one. Next, we outline potential future research directions within this paradigm that can either unlock new use cases or make the paradigm more efficient.

==> Sources/approxedge.tex <==
% \section{approximate computing in edge}\label{sec:approxedge}
% /////// RESUME HERE ///////


% [Edge-Supported Approximate Analysis for Long Running Computations]
% With more and more IoT devices being readily available and used throughout one's daily lives, it is important for data analytics to be able to properly collect such large scale data and process its information in the most efficient way to return optimal results. The summarization of an edge-supported approximation techniques proposed in the outlined paper as well as an educated criticism on the
% approach the authors used. In the mentioned paper, the author’s main objective was to demonstrate the use of approximation techniques applied to data collected at the edge of a network to adequately process this information and reduce any computational resource requirements. The decision to use these approximation techniques were due to the fact that these techniques simplify the overall analysis workflow to reach a particular outcome. Moreover, the advantages of reduced execution times and reduced requirements on the computation infrastructure were a major contributing factor in taking such approach. The approximation techniques used when ANN was not available are ranked from most to least contribution as such: parameter interval reduction, parameter value skipping, and finally loop reduction.

% Some of the approximation techniques proposed in the paper included: (1) loop reduction - a method where during a simulation the number of loop iterations are reduced, in return the total execution time is minimized and yields a reduced computational overhead. (2) artificial neural network - a method where the used of historical data is used to train a system and discover patterns within a simulation (EnergyPlus experiment). Moreover, the data is used as a function approximator to predict certain behaviors of the simulation. (3) memory access skipping - most viable technique used, patterned based method that skips certain tasks during a simulation to decreases the amount of attempts to access memory. IoT devices are typically connected to the same network and generate large amounts of data. The problem associated with such instance is what portion of that generate data is considered to be relevant/useful and how much data should be transfer and stored within cloud based data centers. Here the idea of edge-computing isconsiderably useful because the only data being processed is the data generated at the very edge of the network. Such practice allows for the implementation of various computational approximation techniques to further analyze the captured data and make use of it.

% The goal of this study was determine the best approach to optimize the energy usage in buildings. This study serves as the perfect test bench senecio because smart building are equip with many data sensors that generate pertinent amounts of data that ultimately helps with the overall optimality and function of that specific building. To test the proposed idea, the authors assumed the fact that multiple building would be requesting optimal energy consumptions so they would have to evenly distribute the requests (jobs) amongst there cloud federation. Four strategies were taken under consideration (1) Traditional - only resources providers were able to perform computations (2) Edge - data centers position at the edge of the network could contribute to the computations of collect data (3) Approximation - using approximation techniques resources provides can perform computations when the needs of the SLA was not meet (4) Edge + Approximation - edge resources are able to contribute to the computations using approximation techniques. In an attempt to maximize the number of tasks completed at edge/in-transit resources, the authors discovered that edge-approximation (after the overhead for using an artificial neural network was passed) is the most efficient technique in terms of job acceptance ratio. The edge-approximation technique achieved 100\% job acceptance in the highest scenario, while the edge strategy has 22\% more acceptance than approximation alone. Addition of edge resources in jobs results in more jobs to be executed with higher accuracy. This is fairly impressive and is what the paper sought to prove.

% The criticisms we have in regards to this paper are: (1) the authors assumes an unlimited budget for Amazon resources, so while the maximization of throughput was achieved, minimization of cost (of computation power) was not. (2) For cases where approximation is not available, accuracy is shown to be 100\% which skews results.

% [ApproxIoT: Approximate Analytics for Edge Computing]
% This paper explores an intersection of three important computing technologies: the internet of things (IoT), approximate computing, and edge computing. The Internet of things (IoT) is a method of obtaining data from sensors to make real world observations and analyze trends in real time. For example, Google Maps collects sensor data from Android users to make predictions about traffic and for finding the
% quickest routes. The problem is that there are over one billion active Android phones that are uploading data in the order of zettabytes. Computing most of this data might demonstrate a diminishing return in terms of accuracy and would be a waste of resources.

% To improve the performance of IoT applications, the authors propose ApproxIoT: a new data analytics system that takes advantage of approximate and edge computing. Approximate computing uses algorithms that sacrifice exact calculations in favor of faster throughput and efficiency. The edge is a smaller, less powerful datacenter that can be distributed more throughout a region. In the IoT context, it can be used for organizing data from sensors near it before the central data center requests it for analysis.

% In the ApproxIoT system, sensors will report their individual datastreams to an edge center close by. The nodes on the edge will keep a collection of data entries for each sensor. This collection has a fixed size so when a new data item comes in, the node calculates weights of the substream and replaces an item with the new one. A client can then submit a query to the central datacenter with latency and error constraints. These constraints are then converted to a sample size for each substream. A sampling node on the edge selects items from each substream based another weight calculation. These samples are sent to the central datacenter which can perform a faster analysis due to the filtration of the data from the edge. 

% The authors evaluated their system using test datastreams with both mathematically modelled input rates and real world datasets. They compared it to a sampling algorithm that simply selects at random from substreams. For accuracy loss, it is reported that their system achieved average losses at around 0.035\% across different settings and stream distributions. Even when sampling only 10\% of the arriving data, the loss in accuracy for ApproxIoT was still under 0.05\% while random sampling lost a little over 0.3\%. This means that ApproxIoT is more effective at selecting the most important data.

% Since it can achieve accuracy using less data, the system can increase its
% throughput and handle more requests. This benefit is demonstrated when comparedwith a standard algorithm that analyzes the entire dataset, thus achieving 100\% accuracy. When ApproxIoT samples the entire dataset, its throughput is about equal to the standard algorithm. This shows that ApproxIoT’s sampling algorithm adds no extra stress on the datacenter’s resources.

% The authors provide some suggestions for future work. One is in extending this system to handle more complex queries that may include join operations. The next goal is to implement automatic fine tuning for calculating the sampling size. I would like to see research performed where the sensors themselves can filter their data reporting. In conclusion, the researchers achieved their goals of incorporating edge and approximate computing technologies to assist in the big data processing for IoT applications.


%Energy-Efﬁcient System Design for IoT Devices
%DryadInc: Reusing work in large-scale computations
